Automated Pruning of Polyculture Plants

Polyculture farming has environmental advantages but requires substantially more pruning than monoculture farming. We present novel hardware and algorithms for automated pruning. Using an overhead camera to collect data from a physical scale garden testbed, the autonomous system utilizes a learned Plant Phenotyping convolutional neural network and a Bounding Disk Tracking algorithm to evaluate the individual plant distribution and estimate the state of the garden each day. From this garden state, AlphaGardenSim selects plants to autonomously prune. A trained neural network detects and targets specific prune points on the plant. Two custom-designed pruning tools, compatible with a FarmBot gantry system, are experimentally evaluated and execute autonomous cuts through controlled algorithms. We present results for four 60-day garden cycles. Results suggest the system can autonomously achieve 0.94 normalized plant diversity with pruning shears while maintaining an average canopy coverage of 0.84 by the end of the cycles. For code, videos, and datasets, see https://sites.google.com/berkeley.edu/pruningpolyculture.

==> figures/circle_iou.tex <==
\begin{figure}
    \vspace{0.2cm}
    \centering
    \frame{\includegraphics[width=42mm]{images/KMeans-IoU.png}\includegraphics[width=42mm]{images/BFS-IoU.png}}
    \caption{\textbf{Circle IoU for days 15, 30, 45 of Cycle 2R}. Each of these figures \textbf{K-Means (left), BFS (right)} show average IoU Score by plant type of the method given the ground truth circles. Note that with a highly occluded plant like Raddichio, neither method is able to match ground truth effectively, because of the sparsity of the segmentation mask. }
    \vspace{-0.7cm}
\label{fig:circleiou}
\end{figure}

==> figures/cycle_plants_pruned.tex <==
\begin{table}
\centering
\vspace{0.15cm}
\scalebox{0.85}{
\begin{tabular}{ |p{2cm}||r||r|r|}
 \hline
 Plant Type & Cycle $#$1 & Cycle $#$2 (Left) & Cycle $#$2 (Right) \\
 \hline
 \hline
 Kale0 & 6 & 6 & 6 \\
 \hline
 Kale1 & 6 & 6 & 6 \\
 \hline
 Turnip0 & 6 & 4 & 3 \\
 \hline
 Turnip1 & 6 & 4 & 3 \\
 \hline
 Borage0 & 4 & 6 & 5 \\
 \hline
 Borage1 & 4 & 5 & 5 \\
 \hline 
 SwissChard0 & 3 & 2 & 4 \\
 \hline
 SwissChard1 & 3 & 0 & 3 \\
 \hline 
 GreenLettuce0 & 2 & 0 & 1 \\
 \hline
 GreenLettuce1 & 1 & 0 & 0 \\
 \hline
 RedLettuce0 & 0 & 1 & 1 \\
 \hline
 RedLettuce1 & 0 & 0 & 1 \\
 \hline
 Cilantro0 & 1 & 1 & 0 \\
 \hline
\end{tabular}}
\caption{Garden Cycles: Number of times a plant was chosen to be pruned for both garden cycles. }
\squeeze
\vspace{0.2cm}
\label{table:cycle_pruned}
\end{table}



==> figures/garden_setup.tex <==
\begin{figure}
    \vspace{0.2cm}
    \centering
    % \frame{\includegraphics[width=75mm, clip]{images/scissor_cad.png}}
    \frame{\includegraphics[width=75mm, clip]{images/garden_labeled.png}}
    % \frame{\includegraphics[width=35mm, height=35mm]{images/tool_head.png}}
    \caption{\markp{TODO: Temporary figure meant to diagram the entire AG physical setup. use old intro image, as it is a better photo} \textbf{AlphaGarden Physical Setup} \textbf{A:} Overhead camera. \textbf{B:} Grow lights to monitor the garden after sunset. Lights are on from 5:00 PM - 9:00 PM. \textbf{C:} Universal tool mount (UTM) used for watering and pruning with Z-axis sensors. \textbf{D:} FarmBot OS that allows control over gantry system. \textbf{E:} Six soil sensors are installed within the planter bed. \textbf{Right: } The UTM allows for irrigation and can use either pruning tool. It also has a snake inspection camera and infrared distance sensor.} 
    \vspace{-0.7cm}
\label{fig:setup}
\end{figure}

==> figures/heatmap_keypoints.tex <==
\begin{figure}
    \vspace{0.2cm}
    \centering
    % \begin{minipage}[b]{0.45\linewidth}
    % \frame{\includegraphics[width=\linewidth, clip]{images/larged_heatmap_cilantro.png}}
    % \end{minipage}
    % \begin{minipage}[b]{0.45\linewidth}
    % \frame{\includegraphics[width=\linewidth, clip]{images/points_cilantro.png}}
    % \end{minipage}
    \frame{\includegraphics[width=42mm, clip]{images/larged_heatmap_cilantro.png}}
    \frame{\includegraphics[width=42mm, clip]{images/points_cilantro.png}}
    \caption{Conversion from a raw heatmap of Cilantro leaf centers to points, calculated with the recursive clustering algorithm.}
    \label{fig:heatmap_points}
    \vspace{-0.5cm}
\end{figure}

==> figures/intro_fig.tex <==
\begin{figure}
    \vspace{0.2cm}
    \centering
    \begin{tabular}{c}
    {\frame{\includegraphics[width=80mm, height=32mm]{images/AlphaGarden-sideview.jpg}}}
    \end{tabular}
    % \begin{tabular}{c@{\hspace{2pt}}c@{\hspace{0pt}}}
    % {\frame{\includegraphics[width=30mm, height=30mm]{images/tool_head.jpg}}}&{\frame{\includegraphics[width=54mm, height=30mm]{images/overhead.jpg}}} 84.2mm
    \begin{tabular}{c}
    {\frame{\includegraphics[width=80mm, height=34mm]{images/overhead.jpg}}}
    \end{tabular}
    \caption{\textbf{AlphaGarden.} \textbf{Top:} Physical testbed with the FarmBot gantry system. AlphaGarden includes a custom Rotary Pruner, custom Pruning Shears, a depth sensor, an on-board snake inspection camera, an overhead camera, and soil moisture sensors. %\textbf{Left:} FarmBot universal tool mount with a custom Rotary Pruner, Pruning Shears, depth sensor, and on-board snake inspection camera. 
    \textbf{Bottom:} Overhead image of growth based on two mirrored seed placements for Garden Cycles 3 and 4.}
    \vspace{-0.7cm}
\label{fig:intro}
\end{figure}

==> figures/km_pseudocode.tex <==
\begin{algorithm}
\caption{K-Means bounding disk Tracking Pseucode}\label{alg:cap}
\begin{algorithmic}
    \Procedure{KmeansBoundingDisks}{segmask, s(t-1)}
      \State circles $\gets list()$
      \For{\texttt{$p_i \in s(t-1)$}}
        \State $\text{mask}(p_i)\gets \text{IsolatePlant(p_i, segmask)}$\comment{creates a point cloud of pixels corresponding to plant $p_i$}
        \State $\text{clusters}\gets \text{KMeans(mask(p_i), segmask)}$
        
      \EndFor
      \State \textbf{return} $b$
    \EndProcedure
\end{algorithmic}
\end{algorithm}

==> figures/leaf_cuts.tex <==
\begin{figure}
    \vspace{0.2cm}
    \centering
    \frame{\includegraphics[clip, width=84.2mm]{images/Cuts in a grid.JPG}}
    \caption{\textbf{Examples of Cut types} Images showing complete cut examples using the Pruning Shears and Rotary Pruner \textbf{Top row:} Pruning Shears and leaf before cut;Pruning Shears and leaf after cut; \textbf{Bottom row:} Rotary Pruner and leaf before cut; Pruning Shears and leaf after cut. REMEMBER TO INCLUDE INCOMPLETE CUTS}
    \vspace{-0.7cm}
    
\label{fig:disk}
\end{figure}

==> figures/seed_placement_fig.tex <==
\begin{figure}
    \vspace{0.2cm}
    \centering
    \frame{\includegraphics[width=85mm, clip]{images/seed_placement_1x3.png}}
    \caption{\textbf{VARPOD Seed Placement.} Three seed placements generated by the VARPOD algorithm. The plants are colored by plant type; the voids are colored black. We chose to plant seed placement \#1 for garden cycles 3 and 4.}
    \vspace{-0.7cm}
\label{fig:seed_placement}
\end{figure}
